Convex optimization for the planted k-disjoint-clique problem

We consider the k-disjoint-clique problem. The input is an undirected graph G in which the nodes represent data items, and edges indicate a similarity between the corresponding items. The problem is to find within the graph k disjoint cliques that cover the maximum number of nodes of G. This problem may be understood as a general way to pose the classical `clustering' problem. In clustering, one is given data items and a distance function, and one wishes to partition the data into disjoint clusters of data items, such that the items in each cluster are close to each other. Our formulation additionally allows `noise' nodes to be present in the input data that are not part of any of the cliques. The k-disjoint-clique problem is NP-hard, but we show that a convex relaxation can solve it in polynomial time for input instances constructed in a certain way. The input instances for which our algorithm finds the optimal solution consist of k disjoint large cliques (called `planted cliques') that are then obscured by noise edges and noise nodes inserted either at random or by an adversary.

==> Optimality-conditions.tex <==
In this section, we will provide sufficient conditions for optimality of the solution given by \eref{eqn: proposed solution} to the optimization problem (\ref{eqn: k-clique relaxation}).
We begin by stating the main theorem for this section which follows immediately from the Karush-Kuhn-Tucker conditions for a semidefinite program.

\begin{theorem} \label{thm: KKT conditions}
     Let $X^*$ be feasible for (\ref{eqn: k-clique relaxation}).
     Suppose also that there exists $\blambda \in \R^N_+$, $\mu \in \R$, $\boldeta \in \R^{N\times N}$
     and $S \in \Sigma_+^N$ such that
     \begin{align}
          - \e\e^T + \blambda \e^T +  \e \blambda^T + \mu I + \sum_{\substack{(i,j) \notin E \\ i \neq j}} \boldeta_{ij} \e_i \e_j^T & = S,   \label{dual feas} \\
          \blambda^T (X \e - \e) & = 0, \label{CS: row sum} \\
          \langle S, X \rangle &= 0.    \label{CS: sdp}
     \end{align}
     Here $\Sigma_+^N$ is the cone of $N \times N$ positive semidefinite matrices,
     $\langle \cdot, \cdot \rangle$ is the trace inner product on $\R^{N\times N}$ defined by
     $$
          \langle Y, Z \rangle = \tr(YZ^T)
     $$
     for all $Y, Z \in \R^{N\times N}$,  $\e_i$ denotes the $i$th column of the identity matrix in $\R^{N\times N}$ for all $i=1,\dots, N$, and $\e$ is the
     all-ones vector in $\R^{N}$.
     Then $X^*$ is an optimal solution of (\ref{eqn: k-clique relaxation}).
\end{theorem}


We wish to apply this theorem to \eref{eqn: proposed solution}.  In order to do so, we need to construct multipliers,
which is the subject of the next subsection.  In the following subsection, we prove the main theorem about
optimality of $X^*$.

